BLINK: Multimodal Large Language Models Can See but Not Perceive

We introduce Blink, a new benchmark for multimodal language models (LLMs) that focuses on core visual perception abilities not found in other evaluations. Most of the Blink tasks can be solved by humans "within a blink" (e.g., relative depth estimation, visual correspondence, forensics detection, and multi-view reasoning). However, we find these perception-demanding tasks cast significant challenges for current multimodal LLMs because they resist mediation through natural language. Blink reformats 14 classic computer vision tasks into 3,807 multiple-choice questions, paired with single or multiple images and visual prompting. While humans get 95.70% accuracy on average, Blink is surprisingly challenging for existing multimodal LLMs: even the best-performing GPT-4V and Gemini achieve accuracies of 51.26% and 45.72%, only 13.17% and 7.63% higher than random guessing, indicating that such perception abilities have not "emerged" yet in recent multimodal LLMs. Our analysis also highlights that specialist CV models could solve these problems much better, suggesting potential pathways for future improvements. We believe Blink will stimulate the community to help multimodal LLMs catch up with human-level visual perception.

==> Tables/ensemble.tex <==
\begin{table}[h]
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{Dataset Name} & \textbf{Acc. with Ensemble} & \textbf{Acc. with Single} & \textbf{Norm. Entropy} \\
\hline
Localization & \textbf{52.23} & 46.96 & 0.614\\
\hline
IQTest & \textbf{22.74} & 21.74 & 0.654\\
\hline
DreamSim & \textbf{71.96} & 54.24 & 0.589\\
\hline
Realness & \textbf{45.08} & 25.76 & 0.395\\
\hline
IIW & \textbf{26.12} & 14.55 & 0.286\\
\hline
Correspondence & \textbf{33.43} & 22.38 & 0.392\\
\hline
SpatialRelation & \textbf{48.60} & 32.17 & 0.411\\
\hline
Jigsaw & \textbf{66.33} & 56.00 & 0.724\\
\hline
Depth & \textbf{68.15} & 58.06 & 0.566\\
\hline
ArtStyle & \textbf{80.34} & 65.38 & 0.628\\
\hline
CameraPose & \textbf{54.89} & 49.25 & 0.697\\
\hline
SemanticCorrespondence & \textbf{27.24} & 19.00 & 0.505\\
\hline
FunctionalCorrespondence & \textbf{28.08} & 26.54 & 0.580\\
\hline
Counting & \textbf{52.08} & 42.08 & 0.333\\
\hline
\end{tabular}
\caption {Comparison of accuracy obtained from ensemble vs single predictions across multiple tasks by GPT4V. The table also illustrates the average normalized entropy of predicted results from five runs, which serves as a measure of model uncertainty.}
\label{tbl:ensemble}
\end{table}

==> old/abstract_v0.tex <==
\begin{abstract}


We introduce~\bench, a new benchmark for multimodal language models (LLMs) that focuses on core visual perception abilities not found in other evaluations.
Most of the \bench tasks can be solved by humans ``within a blink'' (\eg, depth estimation, correspondence, and 3D reasoning). However, we find these perception-demanding tasks cast significant challenges for current multimodal LLMs.
% We introduce~\bench, a new benchmark designed to evaluate multimodal large language models (multimodal LLMs) on multiple perception-demanding tasks. 
% This benchmark focuses on core human vision perception abilities missing from existing multimodal LLM benchmarks, like depth estimation, correspondence, and 3D reasoning, emphasizing more nuanced perception understandings of visual data.
% This benchmark presents significant challenges to advanced multimodal large language models (multimodal LLMs), such as GPT-4V(ision) and Gemini, by emphasizing various nuanced perception understanding of visual data.
% We question existing benchmarks only require recognition-level perception, and 
%  We emphasize the need for multimodal LLMs to \textbf{``see'' as humans would do}, by proposing such a benchmark that 
% focuses on \textbf{visual information that is more nuanced than language description}.
% can not be solved using recognition only -- language proxies such as dense image captions. 
\bench is comprised of 3,978 multiple-choice questions paired with single or multiple images and visual prompting, across 14 tasks meticulously selected to be naturally easy for humans and inspired by classical computer vision perception problems. 
While humans get 95.70\% accuracy on average, \bench is surprisingly challenging for existing multimodal LLMs:
even the best-performing GPT-4V and Gemini achieve accuracies of 51.32\% and 45.46\%, only 13.23\% and 7.47\% higher than random guessing, indicating that such perception abilities have not ``emerged'' yet in recent multimodal LLMs.
% In our evaluation on \bench, we benchmarked 16 different models, highlighting a gap of 40\% accuracy achieved by human over the state-of-the-art GPT-4V, indicating significant room for improvement. 
% Our analysis not only highlights the observed limitations of recent multimodal LLMs but also shows 
% Further, the 7B, 13B, and 34B multimodal LLMs perform similarly, indicating that LM scaling (at least in dimensions explored so far) does not help with \bench tasks. 
Our analysis also highlights
that specialist CV models could solve these problems much better, suggesting potential pathways for future improvements. 
 \bench can also serve as a testbed for visual prompting techniques.
We believe \bench will stimulate the community to help multimodal models catch up with human-level perception.
% Project link~\url{https://huggingface.co/PerceptionEval}. \fxy{build page}
 \end{abstract}

==> old/abstract_v1.tex <==



We introduce~\bench, a new benchmark for multimodal language models (LLMs) that focuses on core visual perception abilities not found in other evaluations.

Most of the \bench tasks can be solved by humans ``within a blink'' (\eg, depth estimation, correspondence, and 3D reasoning). However, we find these perception-demanding tasks cast significant challenges for current multimodal LLMs
\yushi{because they resist mediation through natural language}.
% We introduce~\bench, a new benchmark designed to evaluate multimodal large language models (multimodal LLMs) on multiple perception-demanding tasks. 
% This benchmark focuses on core human vision perception abilities missing from existing multimodal LLM benchmarks, like depth estimation, correspondence, and 3D reasoning, emphasizing more nuanced perception understandings of visual data.
% This benchmark presents significant challenges to advanced multimodal large language models (multimodal LLMs), such as GPT-4V(ision) and Gemini, by emphasizing various nuanced perception understanding of visual data.
% We question existing benchmarks only require recognition-level perception, and 
%  We emphasize the need for multimodal LLMs to \textbf{``see'' as humans would do}, by proposing such a benchmark that 
% focuses on \textbf{visual information that is more nuanced than language description}.
% can not be solved using recognition only -- language proxies such as dense image captions. 
\bench is comprised of 3,978 multiple-choice questions paired with single or multiple images and visual prompting, across 14 tasks meticulously selected to be naturally easy for humans and inspired by classical computer vision perception problems. 
While humans get 95.70\% accuracy on average, \bench is surprisingly challenging for existing multimodal LLMs:
even the best-performing GPT-4V and Gemini achieve accuracies of 51.32\% and 45.46\%, only 13.23\% and 7.47\% higher than random guessing, indicating that such perception abilities have not ``emerged'' yet in recent multimodal LLMs.
% In our evaluation on \bench, we benchmarked 16 different models, highlighting a gap of 40\% accuracy achieved by human over the state-of-the-art GPT-4V, indicating significant room for improvement. 
% Our analysis not only highlights the observed limitations of recent multimodal LLMs but also shows 
% Further, the 7B, 13B, and 34B multimodal LLMs perform similarly, indicating that LM scaling (at least in dimensions explored so far) does not help with \bench tasks. 
Our analysis also highlights
that specialist CV models could solve these problems much better, suggesting potential pathways for future improvements. 
 \bench can also serve as a testbed for visual prompting techniques.
We believe \bench will stimulate the community to help multimodal models catch up with human-level perception.
% Project link~\url{https://huggingface.co/PerceptionEval}. \fxy{build page}
 

==> old/abstract_v3.tex <==

The recent discourse around multimodal large language models (LLMs) and their perceptual capabilities has diverged from computer vision's original ambitions of achieving human-level perception through the interpretation of 3D scenes and understanding complex visual properties.
Recent benchmarks, though important, conflate domain knowledge—\ie, having prior knowledge about clinical radiology or history—with perceptual capability.
Our experiments find that this conflation reductively evaluates perception through dense captioning; replacing the image with a task-agnostic dense caption for blind-GPT4 performs very well on them.
In response, we introduce \bench, a new benchmark designed to realign with the foundational goals of computer vision by presenting tasks that require perception beyond mere dense captioning.
\bench reformats 14 classic computer vision tasks, including depth estimation, semantic correspondence, multi-view reasoning, visual IQ, forensics, and much more, into 3,978 multiple-choice questions for evaluating multimodal LLMs.
While humans get 95.70\% accuracy on average, the best-performing GPT-4V and Gemini models achieve accuracies of 51.32\% and 45.46\%, only 13.23\% and 7.47\% higher than random guessing.
Our analysis also highlights that specialist vision models could solve these problems much better, suggesting potential pathways for future improvements for multimodal LLMs. 
% We believe \bench will stimulate the community to help multimodal models catch up with human-level perception.




 



==> old/intro_v1.tex <==
\section{Introduction}
\label{sec:intro}



Multimodal Large Language Models (LLMs) ~\cite{gpt4, gemini, chen2023palix, liu2024visual, liu2023improved, bai2023qwenvl, wang2023cogvlm, dai2023instructblip, chen2023sharegpt4v, internlmxcomposer2, lu2023unified} have recently garnered unprecedented worldwide attention due to their superior performance across a broad spectrum of tasks and domains.  
%For instance, in the realm of vision and language, large generative models are capable of producing stunning outputs (\eg, high-quality images, coherent videos, comprehensive text descriptions) at speeds orders of magnitude faster than their human counterparts. \yushi{MLLMs live in a different world from Diffusion models. I suggest removing the prior sentence}
Their ability to ``understand'' images and texts has the potential to revolutionize multiple fields, such as robotics~\cite{driess2023palm, google2024pivot}, medicine~\cite{singhal2023towards, thirunavukarasu2023large}, and education~\cite{bewersdorff2024taking}. 
%The related tools have been integrated into people's daily workflow and have shown the potential to revolutionize multiple fields, such as robotics~\cite{driess2023palm, google2024pivot}, medicine~\cite{singhal2023towards, thirunavukarasu2023large}, and education~\cite{bewersdorff2024taking}.
However, despite the great promise, existing multimodal LLMs sometimes still fall short in certain surprisingly simple situations -- they may struggle to interpret the structure or shading of the scene; and they may even fail to conduct naive pattern matching! 
\yushi{Do we need to cite something here? Hard to find because no one has evaluated on these tasks... Another option is to say old things like spatial relations and counting. But these are not surprising.}
\fxy{as we will show later in this paper?} 
%they may struggle to interpret the structure or shading of the scene even though they can effectively generate them.
% %(\weichiu{is there a better example here?})
This makes one ponder: to what extent do these models understand what they see? What do they know about our visual world? And how far are they from human visual perception?


To shed light on these questions, researchers have developed a surge of benchmarks to evaluate the effectiveness of multimodal LLMs across a wide array of visual tasks, such as optical character recognition (OCR), object/scene (attribute) recognition, visual reasoning \fxy{(object usage)}, \fxy{(human)} relation prediction, etc.~\cite{liu2023mmbench, li2023seed, li2023seed2, yue2023mmmu, lu2023mathvista, liu2023visual, liu2023hidden}
%and even college exams.
Unfortunately, while these tasks provide insights into the behavior of the models across various dimensions, most of them still focus primarily on evaluating the \emph{visual recognition} capabilities of multimodal LLMs and the domain knowledge they encode. 
In fact, \yushi{as prior work~\cite{yang2022empirical, hu2022promptcap, berrios2023towards} and} our experiments in \S\ref{sec:exp_analysis} suggest, many of these previous benchmarks can be easily addressed by first generating task-agnostic dense captions, followed by feeding these captions into LLMs to query for answers.
However, an image is worth a thousand words; it carries rich information that often surpasses language description \fxy{bottlenecks}. 
Moreover, human visual perception encompasses a diverse set of capabilities, beyond simple recognition.
We can effortlessly perform pattern matching and grouping within or across images. 
We are also able to discern the (coarse) geometry and composition of a scene. 
The design and focus of current benchmarks thus limit our ability to effectively measure the visual perception gap between humans and machines.


\begin{figure}[t]
    \centering    
    \includegraphics[width=0.95\textwidth]{figures/comparison.pdf}
    \caption{\textbf{Comparison between \bench and previous benchmarks. \nascomment{I think you need citations here, both for previous benchmarks and for the sources of the blink tasks}}}
    \label{fig:intro-difference}
\end{figure}



With these motivations in mind, we propose \texttt{BLINK}, a new benchmark to faithfully evaluate the visual perception capability of multimodal LLMs. 
\texttt{BLINK} consists of 14 classic computer vision tasks, ranging from low-level pattern matching (\eg, visual correspondence) to high-level visual understanding (\eg, visual similarity). 
We recast each task as a question-answering problem, 
%Each task consists of a number of question-answering pairs, 
where the choices can be images or texts, the questions may contain multiple images, and the prompts could be both textual and visual.
The tasks are meticulously selected such that they are difficult to solve by generic captioning approaches; instead, the models are forced to comprehend both the text and the image(s) jointly.  
The benchmark features a diverse set of images curated from a wide range of datasets~\cite{lin2014microsoft, krishna2016visual, bell14intrinsic, hpatches_2017_cvpr,chen2016single, gupta2019lvis, fu2023dreamsim, fu-etal-2022-theres}, encompassing indoor household scenes as well as outdoor urban or natural environments. 
The textual questions and choices are either derived from the datasets, or manually written by humans. 
\yushi{Say something about visual prompts? The visual prompts allow us to recast pixel-level tasks like correspondence and depth estimation into multiple-choice question answering.}
The heterogeneous structure allows us to effectively 
evaluate a much more diverse and fine-grained set of visual perception capabilities.
On average, each question can be solved by a human within a blink of an eye (\ie, within a few seconds), hence the name \texttt{BLINK}.


We carefully evaluate 16 multimodal LLMs with various sizes (\ie, 7B, 13B, 34B) on \texttt{BLINK}. We observe the paradox that while these problems are easy for humans\fxy{(95.70\%)}, they are extremely hard for existing machinery -- even the most powerful state-of-the-art GPT-4V model can only achieve 51.32\% accuracy on average, which is \textcolor{red}{44.38\%} worse than humans, 
% \textcolor{red}{xx} worse than specialist models, 
and 13.23\% better than random guessing. 
% To validate whether scaling can mitigate the perception gap, we further compare open-sourced multimodal LLMs of various sizes, finding that their performance on \texttt{BLINK} is similar.
We also experiment with specialist CV models and find that they perform much better than multimodal LLMs. For example, the specialist outperforms GPT-4V by 62.8\% on correspondence, 38.7\% on depth estimation, and 34.6\% on multi-view reasoning.
Our experimental results suggest not only that many visual perception abilities have not yet ``emerged'' in current multimodal LLMs, but also highlight the need to rethink different approaches to fully unlock their multimodal potentials. 
We believe our benchmark, \texttt{BLINK}, can serve as an effective testbed for bridging the gap between the remarkable generative capabilities of multimodal LLMs and human perceptual abilities.

In summary, we make the following contributions:
\begin{enumerate}
    \item We collect \bench, which includes 3,9K questions and 7.3K images covering 14 diverse perception-demanding tasks, including newly introduced tasks and inherited ones from traditional computer vision problems.
    \item We evaluate 16 most recent MLLMs on \bench and show that our benchmark presents formidable challenges to existing methods: the most powerful GPT-4V model performs 43.65\% worse than the average human in our experiments and only 13.23\% better than a random guess, shedding light to future researches.
    \item We explore \bench and provide an comprehensive set of in-depth analysis, showing that: a) language proxies such as dense image captions are less useful on our benchmark versus others; b) different visual prompting can affect multimodal LLMs behaviors; c) specialist computer vision models can do much better than multimodal LLMs.
\end{enumerate}

==> old/intro_v2_ranjay.tex <==
\section{Introduction}
\label{sec:intro}


Compared to today, computer vision was originally defined in opposition to pattern recognition~\cite{do1961machine}. 
Pioneers were attempting to interpret images as projections of 3D scenes, not 2D arrays of flat ``patterns''~\cite{minsky1969introduction,marr2010vision}.
Because 3D representation and reconstruction quickly proved to be too difficult, early researchers defined a number of intermediate tasks towards achieving human-level perception:
They focused on understanding optical properties like reflectance~\cite{wang1993layered,black1993framework}, 3D primitives through multi-view reasoning~\cite{marr1976cooperative,hartley2003multiple}, geometric reasoning through depth estimation~\cite{torralba2002depth}, instance recognition through semantic correspondence~\cite{lowe1999object},  affordance through keypoint grounding~\cite{harris1988combined}, forensics through intrinsic images~\cite{barrow1978recovering}.
For example, 3D primitives like relative camera pose estimation required machines to localize keypoints across multi-view images. \nascomment{maybe need a transition here since the idea in the next sentence really takes a 2024 perspective; I don't think anyone would have made this point five or ten years ago.  (I could be wrong, I don't know all this history!  but I don't think natural language was thought about much in CV until recently)}
A common theme amongst all of these tasks lies in the difficulty of expressing the intermediate stages of reasoning in language. Even referring to individual keypoints in language becomes a challenge due to its imprecision \nascomment{maybe restate as ``Natural language is not well suited to some operations, e.g., referring to keypoints, because it is by nature imprecise.''}.
Yet in the modern era of large language models, we, as a community, have diminished computer vision to simply pattern matching for language tasks~\cite{gpt4, gemini, chen2023palix, liu2024visual, liu2023improved, bai2023qwenvl, wang2023cogvlm, dai2023instructblip, chen2023sharegpt4v, internlmxcomposer2, lu2023unified}. \nascomment{last sentence is really quite strong and might irritate some readers.  maybe make it a bit less direct, like pose it as a question ``have we diminished ...?'' or find a quote from someone else so the attack isn't coming from this paper's authors directly?}



This paper is a re-centering of the community's original goals through a quantitative benchmark for this modern era. \nascomment{slightly grandiose -- maybe say ``This paper aims to recenter the computer vision community's original goals through a quantitative benchmark that responds to modern models''}
To appropriately position the benchmark, let's revisit how we currently evaluate perception through using multimodal large language models~\cite{liu2023mmbench, li2023seed, li2023seed2, yue2023mmmu, lu2023mathvista, liu2023visual, liu2023hidden}. 
While many of these benchmarks have been popularized as the de~facto evaluation measures for influential models like GPT4V and Gemini-Pro, they conflate perception with domain knowledge.
At the risk of singling out one benchmark, let's consider questions highlighted in the popular MMMU benchmark~\cite{yue2023mmmu}:
``In the political cartoon, the United States is seen as fulfilling which of the
following roles? <image 1>'' and ``You are shown subtraction <image 1>, T2 weighted <image 2> and T1 weighted axial <image 3> from a screening breast MRI. What is the
etiology of the finding in the left breast?''. The first conflates perception with political roles and the second with clinical radiology.
While MMMU and other benchmarks are still vital contributions \nascomment{be more precise here, it sounds insincere.  why are they vital?}, such conflation has also been reported for past benchmarks by others~\cite{yang2022empirical, hu2022promptcap, berrios2023towards}. Our experiments  show that this conflation reductively evaluates perception as a dense captioning task. In other words, \textbf{by replacing the image with a task-agnostic dense caption, our experiments show that a blind-GPT4 performs well on these ``multimodal tasks''.}




\begin{figure}[t]
    \centering    
    \includegraphics[width=0.95\textwidth]{figures/comparison.pdf}
    \caption{\textbf{Comparison between \bench and previous benchmarks. \nascomment{I think you need citations here, both for previous benchmarks and for the sources of the blink tasks}}}
    \label{fig:intro-difference}
\end{figure}




In response, we propose \bench. \bench reimagines traditional computer vision goals through a format that allows us to evaluate multimodal LLMs.
\texttt{BLINK} consists of 14 classic computer vision tasks, ranging from low-level visual correspondences, depth estimation, multi-view reasoining, visual IQ tests, and many others.
It contains $3.9$K questions across $7.3$K images.
The images tasks are meticulously selected such that they are difficult to solve by reducing the evaluation using dense captioning; instead, the models must perceive the contents of the image(s) to answer.  
We recast each traditional task into a modern question-answering format, where answer choices are either images or text. 
Questions may contain multiple images, curated from a wide range of datasets~\cite{lin2014microsoft, krishna2016visual, bell14intrinsic, hpatches_2017_cvpr,chen2016single, gupta2019lvis, fu2023dreamsim, fu-etal-2022-theres}, encompassing indoor household scenes as well as outdoor urban or natural environments.
The textual questions and choices are either derived from the datasets, or manually written by humans. 
On average, each question can be solved by a human subject within a \bench of an eye.





We carefully evaluate 16 multimodal LLMs with various sizes (\ie, 7B, 13B, 34B) on \texttt{BLINK}. We observe the paradox that while these problems are easy for humans (\textcolor{red}{$95.70\%$} average accuracy), they are extremely hard for existing machinery–even GPT-4V model can only achieve $51.32\%$ accuracy on average, which is \textcolor{red}{$44.38\%$} worse than humans, 
and 13.23\% better than random guessing. 
% To validate whether scaling can mitigate the perception gap, we further compare open-sourced multimodal LLMs of various sizes, finding that their performance on \texttt{BLINK} is similar.
We also experiment with specialist vision models and find that they perform much better than multimodal LLMs. For example, the specialist outperforms GPT-4V by $62.8\%$ on correspondence, $38.7\%$ on depth estimation, and $34.6\%$ on multi-view reasoning.
Our experimental results suggest not only that we have been overestimating the perceptual capabilities of multimodal LLMs, but that perhaps they can learn from existing specialist models that already possess such capabilities~\cite{hu2023visual}.
We believe \bench can serve as an effective testbed for bridging the gap traditional notions of perception with the modern generative capabilities of multimodal LLMs.
\yushi{say absolute or relative improvement}


% We explore \bench and provide an comprehensive set of in-depth analysis, showing that: a) language proxies such as dense image captions are less useful on our benchmark versus others; b) different visual prompting can affect multimodal LLMs behaviors; c) specialist computer vision models can do much better than multimodal LLMs.
% We explore \bench and provide an comprehensive set of in-depth analysis, showing that: a) language proxies such as dense image captions are less useful on our benchmark versus others; b) different visual prompting can affect multimodal LLMs behaviors; c) specialist computer vision models can do much better than multimodal LLMs.

==> old/intro_v3.tex <==
\section{Introduction}
\label{sec:intro}


% Compared to today, computer vision was originally defined in opposition to pattern recognition~\cite{do1961machine}. 
% Pioneers were attempting to interpret images as projections of 3D scenes, not 2D arrays of flat ``patterns''~\cite{minsky1969introduction,marr2010vision}.
% Because 3D representation and reconstruction quickly proved to be too difficult, early researchers defined 

In the quest for achieving human-level perception in computer vision, researchers have developed a series of intermediate tasks:
they focused on understanding optical properties like reflectance~\cite{wang1993layered,black1993framework}, 3D primitives through multi-view reasoning~\cite{marr1976cooperative,hartley2003multiple}, geometric reasoning through depth estimation~\cite{torralba2002depth}, instance recognition through semantic correspondence~\cite{lowe1999object},  affordance through keypoint grounding~\cite{harris1988combined}, forensics through intrinsic images~\cite{barrow1978recovering}.
Recently, inspired by the success of large language models (LLMs), people have started to build multimodal LLMs that aim for superior performance across a broad spectrum of tasks and domains~\cite{gpt4, team2023gemini, bai2023qwenvl, wang2023cogvlm, dai2023instructblip, chen2023sharegpt4v, internlmxcomposer2, lu2023unified}.
These models have achieved success across many vision-language tasks.
However, an image is worth a thousand words. Natural language is not well suited to some operations, \eg, referring to individual keypoints, because of the natural imprecision of language. 
Many core human visual perception abilities are not measured in existing multimodal LLM evaluations because they are difficult to be expressed by language.
This makes one ponder: can multimodal LLMs understand what they see, beyond simple pattern matching with language? Can they tackle the classical computer vision problems that are hard to mediate through language? And how far are they from human visual perception?


This paper aims to recenter the computer vision community's goals on visual perception through a quantitative benchmark that responds to modern multimodal LLMs.
To appropriately position the benchmark, let's revisit how we currently evaluate perception through using multimodal LLMs~\cite{liu2023mmbench, li2023seed, li2023seed2, yue2023mmmu, lu2023mathvista, liu2023visual, liu2023hidden}. 
While many of these benchmarks have been popularized as the de~facto evaluation measures for influential models like GPT4V and Gemini-Pro, they conflate perception with language knowledge and reasoning.
At the risk of singling out one benchmark, let's consider questions highlighted in the popular MMBench~\cite{liu2023mmbench}:
``<image 1> Why is this hummingbird called ruby-throated?'' and ``<image 1> What will happen next? A: the person is gonna laugh B: the person is gonna cry''. For the first question, the vision subpart is to recognize the hummingbird. For the second, it only needs a coarse description of the image. Everything else is left to the language model to solve.
While MMBech and other benchmarks are still important contributions, such conflation has also been reported for past benchmarks by others~\cite{yang2022empirical, hu2022promptcap, berrios2023towards}. Our experiments show that this conflation reductively evaluates perception as a dense captioning task. In other words, \textbf{by replacing the image with a task-agnostic dense caption, our experiments show that a ``blind'' GPT4 performs well on these ``multimodal tasks''.}




\begin{figure}[t]
    \centering    
    \includegraphics[width=0.95\textwidth]{figures/comparison.pdf}
    \caption{\textbf{Comparison between \bench and previous benchmarks. \nascomment{I think you need citations here, both for previous benchmarks and for the sources of the blink tasks}}}
    \label{fig:intro-difference}
\end{figure}




In response, we propose \bench. \bench reimagines traditional computer vision goals through a format that allows us to evaluate multimodal LLMs.
\texttt{BLINK} consists of 14 classic computer vision tasks, ranging from low-level visual correspondences, depth estimation, multi-view reasoining, visual IQ tests, and many others.
It contains $3.9$K questions across $7.3$K images.
The images tasks are meticulously selected such that they are difficult to solve by reducing the evaluation using dense captioning; instead, the models must perceive the contents of the image(s) to answer.  
We recast each traditional task into a modern question-answering format, where answer choices are either images or text. 
Questions may contain multiple images, curated from a wide range of datasets~\cite{lin2014microsoft, krishna2017visual, bell14intrinsic, hpatches_2017_cvpr,chen2016single, gupta2019lvis, fu2023dreamsim, fu-etal-2022-theres}, encompassing indoor household scenes as well as outdoor urban or natural environments.
The textual questions and choices are either derived from the datasets, or manually written by humans. 
On average, each question can be solved by a human subject within a \bench of an eye.





We carefully evaluate 16 multimodal LLMs with various sizes (\ie, 7B, 13B, 34B) on \texttt{BLINK}. We observe the paradox that while these problems are easy for humans (\textcolor{red}{$95.70\%$} average accuracy), they are extremely hard for existing machinery–even GPT-4V model can only achieve $51.32\%$ accuracy on average, which is \textcolor{red}{$44.38\%$} worse than humans, 
and 13.23\% better than random guessing. 
% To validate whether scaling can mitigate the perception gap, we further compare open-sourced multimodal LLMs of various sizes, finding that their performance on \texttt{BLINK} is similar.
We also experiment with specialist vision models and find that they perform much better than multimodal LLMs. For example, the specialist outperforms GPT-4V by $62.8\%$ on correspondence, $38.7\%$ on depth estimation, and $34.6\%$ on multi-view reasoning, in terms of absolute accuracies.
Our experimental results suggest not only that we have been overestimating the perceptual capabilities of multimodal LLMs, but that perhaps they can learn from existing specialist models that already possess such capabilities~\cite{hu2023visual}.
We believe \bench can serve as an effective testbed for bridging the gap traditional notions of perception with the modern generative capabilities of multimodal LLMs.


% We explore \bench and provide an comprehensive set of in-depth analysis, showing that: a) language proxies such as dense image captions are less useful on our benchmark versus others; b) different visual prompting can affect multimodal LLMs behaviors; c) specialist computer vision models can do much better than multimodal LLMs.
% We explore \bench and provide an comprehensive set of in-depth analysis, showing that: a) language proxies such as dense image captions are less useful on our benchmark versus others; b) different visual prompting can affect multimodal LLMs behaviors; c) specialist computer vision models can do much better than multimodal LLMs.

==> sections/8-old-intro.tex <==

\section{Old Introduction -- obsolete}
\label{sec:intro}


Recent multimodal large language models (MLLMs;~\cite{gpt4, gemini, chen2023palix, liu2023visual, bai2023qwenvl, wang2023cogvlm, dai2023instructblip, chen2023sharegpt4v, internlmxcomposer2}) have shown competitive performance in multiple vision and language tasks. These models have the potential to serve humans as AI assistants in multimodal real-world scenarios, on tasks like GUI navigation~\cite{yan2023gpt4vgui} and robotics~\cite{wake2023gpt4vrobotics}. 
Applications like robotic controls~\cite{google2024pivot} require these models to ``see the world'' as humans do, e.g. multi-view reasoning, finding correspondence, and estimating depth. However, rigorous evaluation of these advanced perception abilities is not yet available. \\


Current MLLMs are evaluated on vision-language benchmarks~\cite{liu2023mmbench, li2023seed, li2023seed2, yue2023mmmu, lu2023mathvista} and visual question answering (VQA) tasks~\cite{antol2015vqa, goyal2017making, marino2019ok}. Prior work~\cite{yang2022empirical, hu2022promptcap, berrios2023towards} shows that many of these tasks can be solved through the lens of language, i.e., first describe images with detailed captions, OCR, tags, and attributes, and then feed in these language descriptions to a text-only LLM. 
% As such, these tasks only require recognition-level perception from the visual side, and leave the hard reasoning part to the language sub-model.
However, many fundamental and non-linguistic computer vision tasks are missing from the current MLLM evaluation, for example, correspondence, depth estimation, multi-view reasoning, etc. \yushi{ add more citations?} \nascomment{yes but also try to make this list a bit more comprehensive and don't end it with ``etc.''} The perception abilities to solve these tasks have been proven to be vital for human vision perception \nascomment{this is clunky and circular ... ``perception abilities are vital for perception?''  I'd advise minimizing analogies to human visual processing and instead focus on real-world scenarios where these abilities will be needed for systems (not humans)}, and thus also important for MLLMs to be helpful in diverse real-world scenarios.
Furthermore, with a benchmark that performs a more comprehensive evaluation of MLLMs' visual perception abilities, we can gain more insights into the visual subparts of current MLLMs. For example, such evaluation might help analyze whether an MLLM is bottlenecked by the limited ``sights'' from current image-embedding-as-LM-prefix structures, or by the scale of the language model subpart.\\
% \fxy{They cannot help to tell whether the improvements in recent MLLMs such as GPT-4V are brought by the superiority of their language model subparts or the visual subparts -- considering that multi-modal performance can get boosted by replacing the language subpart with a more powerful model.
% With a benchmark that examines MLLMs' perception abilities beyond recognition, we will be able to gain more insights into current multimodal model structures -- whether they lose visual details and suffer from limited ``sights" from current image-embedding-as-LM-prefix structures.}\\ 

\begin{figure}[t]
    \centering    
    \includegraphics[width=0.95\textwidth]{figures/comparison.pdf}
    \caption{\textbf{Comparison between \bench and previous benchmarks. \nascomment{I think you need citations here, both for previous benchmarks and for the sources of the blink tasks}}}
    \label{fig:intro-difference}
\end{figure}


To systematically and qualitatively \nascomment{quantitatively?} measure the visual perception abilities of MLLMs, we introduce \bench, which specifically tests whether MLLMs can ``see'' as humans do. The goal of this benchmark is to include questions that require more than simple recognition from the visual side, inspired by classical computer vision problems.
As shown in \Cref{fig:teaser}, we manually select 14 perception-demanding tasks requiring 
humans or machines to \textbf{look at the image pixels} to answer, and which cannot  be captured well with language descriptions like captions, OCR, or tags.
Detailed motivation, applications, and the curation process of each task are in \S\ref{sec:data_collect}.
% \bench covers diverse images from multiple resources in the wild, spanning indoor to outdoor scenes, from object centric to scenaries. 
The perception requirements vary from pixel-level, to crop-level, and finally to whole image-level, ranging between semantic and geometric understanding. We select different categories of problems in our benchmark set based on the perception requirements. The full list of tasks is shown in Figure \ref{fig:dataset-circular}.\\

The design principles of \bench are illustrated in \Cref{fig:intro-difference}. \bench has several important and novel points different from existing benchmarks:
\begin{itemize}
    \item \textbf{Visual prompting}: Compared to pure text prompting in existing benchmarks, we include diverse formats of visual prompting in \bench, e.g., we highlight local regions on the images to ask questions about; This enables us to evaluate MLLMs' fine-grained understanding of images.
    \item \textbf{Beyond recognition}: As discussed above, \bench evaluates a diverse set of perception abilities beyond recognition, for example, the MLLM's ability to conduct 3D reasoning or reflectance estimation.
    \item \textbf{``Visual commonsense'' that does not require domain knowledge}: the questions in \bench do not require any domain knowledge or experts to answer, and are commonsense-level easy. Humans are able to answer with a short glance of one second or two in average. \nascomment{if you didn't actually measure (and report in the paper!) human response times, don't make this claim}
    \item \textbf{Interleaved image-text formats}: We provide different formats of image question pairs, including multiple images as choices, multiple images in the question, and multiple choices highlighted in the images.
    \item \textbf{Diverse image sources}: \bench includes in-the-wild images from multiple sources, spanning indoor to outdoor scenes, from object-centric to scenaries, between abstract diagrams, synthesized images, and real photos.
\end{itemize}


% $\hookrightarrow$ 1). visual prompting: Compared to pure text prompting in existing benchmarks, we include diverse formats of visual prompting in \bench, e.g. we highlight local regions on the images to ask questions about; \\
% $\hookrightarrow$ 2). interleaved image-text formats: we provide different formats of image question pairs, including multiple images as choices, multiple images in the question, and multiple choices highlighted in the images.\\
% $\hookrightarrow$ 3). no domain-knowledge required: the questions in \bench do not require any domain knowledge or experts to answer, and are commonsense-level easy. Humans are able to answer with a short glance of one second or two in average; \\
% $\hookrightarrow$ 4). diverse image sources: \bench includes in-the-wild images from multiple sources, spanning indoor to outdoor scenes, from object centric to scenaries, between abstract diagrams, image synthesis, and real photographs. \\

In our experiments, we show the limitations of existing MLLMs on such visual perception demanding tasks.
We experiment with 17 MLLMs and find that, while the 14 tasks in \bench are fairly easy for humans to answer (in average 9x\% \nascomment{update} accuracy), even the most powerful state-of-the-art GPT-4V model could only achieve 50.3\% in average, XX worse than humans, and 12\% better than random guessing. 
These results suggest that many perception abilities have not ``emerged'' in current MLLMs, and the models are unreliable when performing tasks that need these abilities.
Also, the 7B, 13B, and 34B open-sourced MLLMs perform roughly the same, indicating that scaling the language part of MLLMs does not help with \bench tasks. Similar to what prior work~\cite{tong2024eyes} has suggested, we hypothesize that the CLIP-like visual encoders~\cite{radford2021learning} are the bottleneck that limits MLLM's perception ability.\\

Our further analysis shows that language proxies such as dense image captions cannot help models on our benchmark, compared with other benchmarks. Instead, specialist computer vision models can do much better on single tasks than MLLMs. We show how different visual prompting settings such as color change, or box width change, can affect MLLMs' behaviors and attack model robustness. Finally, we include error analysis that can inform future multimodal model development.\\

\textbf{Main Contributions}: Recognizing the need to quantitavely and qualitatively measure how well a MLLM can ``see'' the world, we present \bench, a carefully crafted benchmark designed to explore multiple scales of MLLMs' perception abilities. The major contributions of our work include:
\begin{enumerate}
    \item We collect \bench, which includes 3,978 questions and XXx images covering 14 diverse perception-demanding tasks, including newly introduced tasks and inherited ones from traditional computer vision problems.
    \item We evaluate 17 most recent MLLMs on \bench and show that our benchmark presents formidable challenges to existing methods: the most powerful GPT-4V model performs 40x\% worse than the average human in our experiments and only 12\% better than a random guess, shedding light to future researches.
    \item We explore \bench and provide an comprehensive set of in-depth analysis, showing that: a) specialist computer vision models can do much better than MLLMs; b) different visual prompting can affect MLLMs behaviors; c) language proxies such as dense image captions are less useful on our benchmark versus others.
\end{enumerate}

\nascomment{main issue with intro:  there's no acknowledgment of prior work that created the datasets used to build the benchmark.  right now the language about the relationship to earlier CV benchmarks is too vague.  I strongly suggest making it more clear either that you drew from existing datasets and added something (explain what) OR that you built all of this from scratch, whichever one is correct ...}
